Mask-Based Modeling for Neural Radiance Fields

Most Neural Radiance Fields (NeRFs) exhibit limited generalization capabilities, which restrict their applicability in representing multiple scenes using a single model. To address this problem, existing generalizable NeRF methods simply condition the model on image features. These methods still struggle to learn precise global representations over diverse scenes since they lack an effective mechanism for interacting among different points and views. In this work, we unveil that 3D implicit representation learning can be significantly improved by mask-based modeling. Specifically, we propose masked ray and view modeling for generalizable NeRF (MRVM-NeRF), which is a self-supervised pretraining target to predict complete scene representations from partially masked features along each ray. With this pretraining target, MRVM-NeRF enables better use of correlations across different points and views as the geometry priors, which thereby strengthens the capability of capturing intricate details within the scenes and boosts the generalization capability across different scenes. Extensive experiments demonstrate the effectiveness of our proposed MRVM-NeRF on both synthetic and real-world datasets, qualitatively and quantitatively. Besides, we also conduct experiments to show the compatibility of our proposed method with various backbones and its superiority under few-shot cases.

==> tables/dtu_detail.tex <==
% \resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{2pt}
% \footnotesize
\begin{tabular}{cccccccccccccc}

\toprule 
& & \multicolumn{3}{c}{1-view} & \multicolumn{3}{c}{3-view} &
\multicolumn{3}{c}{6-view} &
\multicolumn{3}{c}{9-view} \\
\cline{3-5}
\cline{6-8}
\cline{9-11}
\cline{12-14}
&  & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS $\downarrow$ 
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS $\downarrow$
& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS $\downarrow$\\ 

& PixelNeRF\cite{yu2021pixelnerf} & \textbf{15.65} &0.532 & 0.540 
 &\textbf{19.24} & 0.685 & 0.400
&\textbf{20.29} & 0.723	& 0.374
 &\textbf{20.91}& 0.748 & 0.350
 \\
& \base & 15.16 & 0.517 & 0.535 & 18.27 & 0.677 & 0.400 & 19.44 & 0.709 & 0.379 & 20.01 & 0.737 & 0.354 \\
& \ourexp & 15.43 & \textbf{0.557} & \textbf{0.492}& 18.67 & \textbf{0.695} & \textbf{0.372} &19.74 & \textbf{0.738} & \textbf{0.341} & 20.41 &\textbf{0.774} & \textbf{0.313}\\
\bottomrule
\end{tabular}
% }

==> tables/rebuttal.tex <==
% \resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{tabular}{@{}lcccc@{}}
\toprule 
 &  1 view & 2 views & 3 views & 5 views  \\ 
 \hline
 \specialrule{0em}{1.5pt}{1pt}   % control space gap
% \cline{1-4}
\base & 27.38 & 28.46 & 28.81 & 29.17\\
\ourexp & \textbf{28.58} & \textbf{29.77} & \textbf{30.20} & \textbf{30.63}\\ 

\bottomrule

\end{tabular}
% }
